Contrastive Learning for Many-to-many Multilingual Neural Machine Translation

Existing multilingual machine translation approaches mainly focus on English-centric directions, while the non-English directions still lag behind. In this work, we aim to build a many-to-many translation system with an emphasis on the quality of non-English language directions. Our intuition is based on the hypothesis that a universal cross-language representation leads to better multilingual translation performance. To this end, we propose mRASP2, a training method to obtain a single unified multilingual translation model. mRASP2 is empowered by two techniques: a) a contrastive learning scheme to close the gap among representations of different languages, and b) data augmentation on both multiple parallel and monolingual data to further align token representations. For English-centric directions, mRASP2 outperforms existing best unified model and achieves competitive or even better performance than the pre-trained and fine-tuned model mBART on tens of WMT's translation directions. For non-English directions, mRASP2 achieves an improvement of average 10+ BLEU compared with the multilingual Transformer baseline. Code, data and trained models are available at https://github.com/PANXiao1994/mRASP2.

==> Tables/category_lang.tex <==
\begin{table}[]
\resizebox{\linewidth}{!}{
\begin{tabular}{l|l|l}
\toprule
              & in PC32                                                                                                      & not in PC32 \\ \hline
in MC24     & \begin{tabular}[c]{@{}l@{}}Bg Cs De El Es \\ Et Fi Fr Gu Hi \\ It Ja Kk Lt Lv \\ Ro Ru Sr Tr Zh\end{tabular} & Nl Pl Pt    \\ \hline
not in MC24 & \begin{tabular}[c]{@{}l@{}}Af Ar Be Eo \\ He Ko Mn Ms \\ Mt My Ka Vi\end{tabular}                            & /           \\ \bottomrule
\end{tabular}
}
\caption{The three categories of languages. We denote them as follows: (i) Group A: languages that are included in both \dataset and \mdataset (ii) Group B: languages that are included in \dataset but not in \mdataset (iii) Group C: languages that are included in \mdataset but not in \dataset }
\label{tab:cat}
\end{table}

==> Tables/del.tex <==
 \toprule
 &
  \multicolumn{2}{c}{\begin{tabular}[c]{@{}c@{}}En-Tr\\ wmt16\end{tabular}} &
  \multicolumn{2}{c}{\begin{tabular}[c]{@{}c@{}}En-Ru\\ wmt19\end{tabular}} &
  \multicolumn{2}{c}{\begin{tabular}[c]{@{}c@{}}En-Fi\\ wmt17\end{tabular}} &
  \multicolumn{2}{c}{\begin{tabular}[c]{@{}c@{}}En-Es\\ wmt13\end{tabular}} &
  \multicolumn{2}{c}{\begin{tabular}[c]{@{}c@{}}En-It\\ wmt09\end{tabular}} &
  \multicolumn{1}{c}{Avg} &
  \multicolumn{1}{c}{$\Delta$} \\
 &
  \multicolumn{1}{c}{$\rightarrow$} &
  \multicolumn{1}{c}{$\leftarrow$} &
  \multicolumn{1}{c}{$\rightarrow$} &
  \multicolumn{1}{c}{$\leftarrow$} &
  \multicolumn{1}{c}{$\rightarrow$} &
  \multicolumn{1}{c}{$\leftarrow$} &
  \multicolumn{1}{c}{$\rightarrow$} &
  \multicolumn{1}{c}{$\leftarrow$} &
  \multicolumn{1}{c}{$\rightarrow$} &
  \multicolumn{1}{c}{$\leftarrow$} &
   &
   \\ 
 \midrule

\baselinea &
  18.2 &
  24.3 &
  17.0 &
  22.6 &
  20.0 &
  28.2 &
  32.8 &
  33.7 &
  29.0 &
  32.0 &
  28.65 &
   \\
%\method  & 18   & 24.5 & 17.3 & 23.1          & 19.9          & 28.2          & 32.7          & 33.8          & 28.9 & 32.0          & 28.63 & -0.02 \\
%\methodx & 20.4 & 20.4 & 18.6 & 23.4 & 22.0 & \textbf{29.4} & 34.1 & 34.3 & 30.4 & 32.6 & 29.69 & +1.04 \\
\methodp &
  \textbf{21.1} &
  \textbf{24.9} &
  \textbf{18.9} &
  \textbf{23.4} &
  \textbf{23.0} &
  \textbf{28.6} &
  \textbf{34.1} &
  \textbf{34.3} &
  \textbf{30.7} &
  \textbf{32.7} &
  \textbf{30.03} &
  \textbf{+1.37} \\
  \bottomrule

==> Tables/extra_zs.tex <==
\begin{table*}[hp]
\begin{center}

\begin{tabular}{lll}
\toprule
           & Fr$\rightarrow$Es & Fr$\rightarrow$De \\
           & wmt13             & wmt19             \\
           \hline
\baselinea & 20.7              & 5.8               \\
\methodb   & 29.1              & 24.1              \\
\method    & 32.1              & 25.9              \\
\bottomrule
\end{tabular}
\caption{Evaluation on representative WMT zero-shot testsets. For Fr$\rightarrow$Es we report de-tokenized BLEU and for Fr$\rightarrow$De we report tokenized BLEU}
\label{tab:extrazs}
\end{center}
\end{table*}

==> Tables/supervised_b.tex <==
\begin{table*}[htb]
\begin{center}
\begin{tabular}{lllllllll|rr}
\toprule
 &
  \multicolumn{2}{c}{\begin{tabular}[c]{@{}c@{}}En-Af\\ opus-100\end{tabular}} &
  \multicolumn{2}{c}{\begin{tabular}[c]{@{}c@{}}En-Be\\ opus-100\end{tabular}} &
  \multicolumn{2}{c}{\begin{tabular}[c]{@{}c@{}}En-Eo\\ opus-100\end{tabular}} &
  \multicolumn{2}{c}{\begin{tabular}[c]{@{}c@{}}En-Ar\\ iwslt2016\end{tabular}} &
  \multicolumn{1}{c}{Avg} &
  \multicolumn{1}{c}{$\Delta$} \\
 &
  \multicolumn{1}{c}{$\rightarrow$} &
  \multicolumn{1}{c}{$\leftarrow$} &
  \multicolumn{1}{c}{$\rightarrow$} &
  \multicolumn{1}{c}{$\leftarrow$} &
  \multicolumn{1}{c}{$\rightarrow$} &
  \multicolumn{1}{c}{$\leftarrow$} &
  \multicolumn{1}{c}{$\rightarrow$} &
  \multicolumn{1}{c}{$\leftarrow$} &
   &
   \\ \hline
\baselinea & 15.7          & 21.8          & 11.2          & 18.1          & 21.1          & 31.7          & 14.0          & 35.3          & 21.11 &       \\
\methodb  & 15.7          & 21.6          & 11.0            & 18            & 20.5          & 32.6          & 14.0            & 35.5          & 21.11 & +0.00          \\
\methodx & \textbf{17.6}          & 24.0            & 12.2          & \textbf{19.5} & \textbf{24.6} & 34.1 & \textbf{15.8} & \textbf{36.6} & 23.05 & +1.94 \\
\method & 17.1 & \textbf{27.7} & \textbf{12.2} & 19.1          & 23.5          & \textbf{34.1} & 15.4          & 35.9          & \textbf{23.13} & \textbf{+2.01}    \\
\bottomrule
\end{tabular}
\caption{\textbf{Group B:} Languages in Group B are included in \dataset but not in \mdataset. We report tokenized BLEU above. For Group B languages, \method brings no BLEU gains nor harm over \methodx. }
\label{tab:supb}
\end{center}
\end{table*}

==> Tables/tatoeba.bak.tex <==
\begin{table*}[t]
\begin{center}
\begin{tabular}{lllllllllll}
\toprule
\multicolumn{11}{c}{Group A}                                                                                                        \\ \hline
Lang       & Fr   & De   & Zh   & Ro   & Cs                   & Tr             & Ru            & Fi   & Es   & It                   \\ \hline
\baselinea & 91.7 & 96.8 & 87.0 & 90.6 & 84.8                & 91.1          & 89.1         & 85.8 & 91.6 & 87.5                \\
\method    & 91.7 & 97.3 & 89.9 & 91.4 & 86.1                & 92.4          & 90.4         & 86.9 & 93.6 & 88.2                \\
\method &
  \textbf{93.0} &
  \textbf{98.0} &
  \textbf{90.7} &
  \textbf{91.9} &
  \textbf{89.3} &
  \textbf{92.4} &
  \textbf{92.3} &
  \textbf{92.4} &
  \textbf{93.5} &
  \textbf{88.9} \\

\hline
 \cline{1-5} \cline{7-11} 

\multicolumn{5}{c}{Group B}            & \multicolumn{1}{c}{} & \multicolumn{4}{c}{Group C}                  & \multicolumn{1}{c}{} \\ \cline{1-5} \cline{7-11} 
Lang       & Af   & Be   & Eo   & Ar   &                      & \multicolumn{2}{l}{Lang}       & Nl   & Pl   & Pt                   \\ \cline{1-5} \cline{7-11} 
\baselinea & 70.8 & 77.0 & 91.3 & 82.3 &                      & \multicolumn{2}{l}{\baselinea} & 25.6 & 6.3  & 37.3                \\
\method    & 76.1 & 80.1 & 92.8 & 84.5 &                      & \multicolumn{2}{l}{\method}    & 35.7 & 14.3 & 46.5                \\
\method &
  \textbf{87.6} &
  \textbf{84.9} &
  \textbf{95.2} &
  \textbf{89.0} &
   &
  \multicolumn{2}{l}{\method} &
  \textbf{60.3} &
  \textbf{28.1} &
  \textbf{58.6} \\
\bottomrule 
\end{tabular}
\caption{\textbf{English-Centric:} Sentence retrieval top-1 accuracy on Tatoeba evaluation set. The reported accuracy is the average of En$\rightarrow$X and X$\rightarrow$En accuracy. For all of the three groups of languages, the accuracy increases as we apply \method. Accuracy further increases using \method. The improvements on Group C are the most significant. }
\label{tab:tatoeba}
\end{center}
\end{table*}

==> Tables/tatoeba_detail.tex <==
\begin{table*}[!tp]
\begin{center}
\resizebox{0.95\linewidth}{!}{
\begin{tabular}{l|ccc||ll|ccc}
\toprule
& \baselinea & \methodb & \method &  &                   & \baselinea & \methodb & \method \\
\midrule
en$\rightarrow$af & 70.2      & 75.9   & \textbf{87.6} &  & en$\rightarrow$ka & 47.1      & 54.6   & \textbf{66.1} \\
af$\rightarrow$en & 71.3      & 76.2   & \textbf{87.5} &  & ka$\rightarrow$en & 48.4      & 52.1   & \textbf{65.5} \\
en$\rightarrow$ar & 81.8      & 83.2   & \textbf{87.9} &  & en$\rightarrow$kk & 40.3      & \textbf{44.7}   & 37.2 \\
ar$\rightarrow$en & 82.7      & 85.7   & \textbf{90.0} &  & kk$\rightarrow$en & 36.9      & \textbf{43.0}   & 40.2 \\
en$\rightarrow$az & 10.1      & 15.0   & \textbf{21.8} &  & en$\rightarrow$ko & 85.4      & 88.5   & \textbf{91.2} \\
az$\rightarrow$en & 5.3       & 14.8   & \textbf{25.3} &  & ko$\rightarrow$en & 88.6      & 89.6   & \textbf{91.8} \\
en$\rightarrow$be & 76.4      & 79.0   & \textbf{83.8} &  & en$\rightarrow$ku & 7.6       & 11.5   & \textbf{13.9} \\
be$\rightarrow$en & 77.5      & 81.1   & \textbf{85.9} &  & ku$\rightarrow$en & 3.2       & 11.5   & \textbf{14.1} \\
en$\rightarrow$bg & 88.7      & \textbf{91.2}   & 90.5 &  & en$\rightarrow$lt & 90.5      & 93.4   & \textbf{95.2} \\
bg$\rightarrow$en & 90.8      & 90.4   & \textbf{93.1} &  & lt$\rightarrow$en & 92.9      & 93.5   & \textbf{95.1} \\
en$\rightarrow$bn & 0.3       & 0.4    & \textbf{15.0} &  & en$\rightarrow$mk & 31.9      & 40.4   & \textbf{58.3} \\
bn$\rightarrow$en & 0.2       & 0.6    & \textbf{14.4} &  & mk$\rightarrow$en & 35.2      & 49.4   & \textbf{66.7} \\
en$\rightarrow$bs & 25.4      & 42.4   & \textbf{59.9} &  & en$\rightarrow$mn & 55.5      & 63.6   & \textbf{73.2} \\
bs$\rightarrow$en & 16.9      & 45.5   & \textbf{66.9} &  & mn$\rightarrow$en & 55.0      & 60.9   & \textbf{75.0} \\
en$\rightarrow$cs & 83.1      & 85.6   & \textbf{87.5} &  & en$\rightarrow$mr & 10.1      & 15.5   & \textbf{22.9} \\
cs$\rightarrow$en & 86.4      & 86.6   & \textbf{91.1} &  & mr$\rightarrow$en & 2.9       & 13.3   & \textbf{25.0} \\
en$\rightarrow$da & 17.8      & 21.3   & \textbf{32.0} &  & en$\rightarrow$nb & 17.8      & 20.3   & \textbf{35.0} \\
da$\rightarrow$en & 8.0       & 19.8   & \textbf{32.9} &  & nb$\rightarrow$en & 12.3      & 20.2   & \textbf{35.0} \\
en$\rightarrow$de & 96.5      & 97.4   & \textbf{97.8} &  & en$\rightarrow$nl & 30.2      & 37.1   & \textbf{58.9} \\
de$\rightarrow$en & 97.0      & 97.1   & \textbf{98.1} &  & nl$\rightarrow$en & 20.9      & 34.3   & \textbf{61.7} \\
en$\rightarrow$el & 79.6      & 81.7   & \textbf{85.2} &  & en$\rightarrow$pl & 9.9       & 15.0   & \textbf{26.4} \\
el$\rightarrow$en & 84.2      & 87.1   & \textbf{89.9} &  & pl$\rightarrow$en & 2.7       & 13.6   & \textbf{29.8} \\
en$\rightarrow$eo & 90.6      & 92.2   & \textbf{94.9} &  & en$\rightarrow$pt & 40.8      & 46.1   & \textbf{55.9} \\
eo$\rightarrow$en & 91.9      & 93.3   & \textbf{95.4} &  & pt$\rightarrow$en & 33.7      & 46.8   & \textbf{61.2} \\
en$\rightarrow$es & 90.3      & \textbf{92.5}   & 91.7 &  & en$\rightarrow$ro & 89.0      & \textbf{91.1}   & 90.5 \\
es$\rightarrow$en & 92.8      & 94.7   & \textbf{95.3} &  & ro$\rightarrow$en & 92.1      & 91.6   & \textbf{93.2} \\
en$\rightarrow$et & 85.4      & 88.0   & \textbf{90.4} &  & en$\rightarrow$ru & 87.9      & 88.8   & \textbf{91.5} \\
et$\rightarrow$en & 89.9      & 90.5   & \textbf{93.5} &  & ru$\rightarrow$en & 90.3      & 91.9   & \textbf{93.1} \\
en$\rightarrow$eu & 7.0       & 9.7    & \textbf{11.2} &  & en$\rightarrow$sk & 16.4      & 23.4   & \textbf{45.2} \\
eu$\rightarrow$en & 1.8       & 6.6    & \textbf{10.4} &  & sk$\rightarrow$en & 6.3       & 21.0   & \textbf{53.1} \\
en$\rightarrow$fi & 84.7      & 85.6   & \textbf{90.0} &  & en$\rightarrow$sl & 17.0      & 23.2   & \textbf{38.2} \\
fi$\rightarrow$en & 86.8      & 88.1   & \textbf{94.7} &  & sl$\rightarrow$en & 8.4       & 20.8   & \textbf{40.5} \\
en$\rightarrow$fr & 91.3      & 91.5   & \textbf{92.5} &  & en$\rightarrow$sq & 9.2       & 11.9   & \textbf{17.6} \\
fr$\rightarrow$en & 92.1      & 91.8   & \textbf{93.4} &  & sq$\rightarrow$en & 3.3       & 9.7    & \textbf{17.1} \\
en$\rightarrow$gl & 37.2      & 37.4   & \textbf{44.2} &  & en$\rightarrow$sr & 82.7      & \textbf{84.7}   & 83.6 \\
gl$\rightarrow$en & 31.9      & 35.9   & \textbf{43.7} &  & sr$\rightarrow$en & 83.3      & 86.2   & \textbf{86.8} \\
en$\rightarrow$he & 69.4      & 72.9   & \textbf{80.6} &  & en$\rightarrow$sv & 16.0      & 17.0   & \textbf{28.8} \\
he$\rightarrow$en & 75.7      & 76.4   & \textbf{84.4} &  & sv$\rightarrow$en & 15.4      & 16.8   & \textbf{27.1} \\
en$\rightarrow$hi & 78.8      & 86.2   & \textbf{92.9} &  & en$\rightarrow$ta & 1.0       & 2.0    & \textbf{19.5} \\
hi$\rightarrow$en & 81.9      & 85.5   & \textbf{95.4} &  & ta$\rightarrow$en & 0.3       & 0.3    & \textbf{19.5} \\
en$\rightarrow$hr & 25.8      & 37.9   & \textbf{54.3} &  & en$\rightarrow$th & 0.9       & 2.2    & \textbf{6.6}  \\
hr$\rightarrow$en & 15.3      & 37.9   & \textbf{60.6} &  & th$\rightarrow$en & 0.4       & 1.3    & \textbf{3.3}  \\
en$\rightarrow$hu & 3.9       & 5.1    & \textbf{10.0} &  & en$\rightarrow$tr & 90.4      & \textbf{91.1}   & 90.8 \\
hu$\rightarrow$en & 1.1       & 4.3    & \textbf{8.3}  &  & tr$\rightarrow$en & 91.7      & 93.6   & \textbf{93.9} \\
en$\rightarrow$hy & 0.4       & \textbf{1.1}    & 0.8  &  & en$\rightarrow$uk & 25.8      & 36.2   & \textbf{50.6} \\
hy$\rightarrow$en & 0.4       & 0.7    & \textbf{0.8}  &  & uk$\rightarrow$en & 24.6      & 37.5   & \textbf{57.0} \\
en$\rightarrow$id & 46.1      & 58.9   & \textbf{69.8} &  & en$\rightarrow$ur & 1.2       & 2.2    & \textbf{2.7}  \\
id$\rightarrow$en & 55.7      & 66.5   & \textbf{76.0} &  & ur$\rightarrow$en & 0.2       & 1.5    & \textbf{2.8}  \\
en$\rightarrow$it & 86.8      & 87.8   & \textbf{88.5} &  & en$\rightarrow$vi & 91.5      & 94.4   & \textbf{95.1} \\
it$\rightarrow$en & 88.2      & 88.5   & \textbf{89.3} &  & vi$\rightarrow$en & 92.1      & 93.5   & \textbf{94.9} \\
en$\rightarrow$ja & 51.1      & \textbf{63.5}   & 52.4 &  & en$\rightarrow$zh & 85.4      & \textbf{89.5}   & 88.9 \\
ja$\rightarrow$en & 39.3      & \textbf{58.7}   & 56.7 &  & zh$\rightarrow$en & 88.6      & 90.3   & \textbf{92.4}    \\
\bottomrule
\end{tabular}
}
\end{center}
\caption{Simiarity search top-1 accuracy on Tatoeba}
\label{tab:tatdetail}
\end{table*}
